Initiation of the detonation in the gravitationally confined detonation model of Type Ia supernovae

We study the initiation of the detonation in the gravitationally confined detonation (GCD) model of Type Ia supernovae (SNe Ia). Initiation of the detonation occurs spontaneously in a region where the length scale of the temperature gradient extending from a flow (in which carbon burning is already occurring) into unburned fuel is commensurate to the range of critical length scales which have been derived from 1D simulations that resolve the initiation of a detonation. By increasing the maximum resolution in a truncated cone that encompasses this region, beginning somewhat before initiation of the detonation occurs, we successfully simulate in situ the first gradient-initiated detonation in a whole-star simulation. The detonation emerges when a compression wave overruns a pocket of fuel situated in a Kelvin-Helmholtz cusp at the leading edge of the inwardly directed jet of burning carbon. The compression wave pre-conditions the temperature in the fuel in such a way that the Zel'dovich gradient mechanism can operate and a detonation ensues. We explore the dependence of the length scale of the temperature gradient on spatial resolution and discuss the implications for the robustness of this detonation mechanism. We find that the time and the location at which initiation of the detonation occurs varies with resolution. In particular, initiation of a detonation had not yet occurred in our highest resolution simulation by the time we ended the simulation because of the computational demand it required. We suggest that the turbulent shear layer surrounding the inwardly directed jet provides the most favorable physical conditions, and therefore the most likely location, for initiation of a detonation in the GCD model.

==> tab1.tex <==
\begin{deluxetable}{rccccc}
\tabletypesize{\footnotesize}
\tablewidth{0pc}
\tablecaption{Detonation conditions \label{tab:conditions}}
\tablehead{ \colhead{Resolution} & \colhead{Time}   & \colhead{Location (x,y)} & \colhead{Fuel Density} & \colhead{$T_{max}$} & \colhead{$T_0$} \\  \colhead{[$10^2$ cm]} &\colhead{[s]}  &    \colhead{  [$10^8$ cm]}  & \colhead{[$10^7$ g cm$^{-3}$]} & \colhead{[$10^9$ K]} & \colhead{[$10^7$ K]} } 
\startdata
4,000    & 2.204 & (0.00,-2.04) & 1.1 & $\sim$3.0 & $\sim$10 \\
   500    & 2.266 & (0.19,-1.95) & 1.2|1.6 & $\sim$3.0 & $\sim$20  \\
   250   &  2.264 & (0.21,-1.97)  & 1.2|1.6 & $\sim$3.0 & $\sim$20 \\
   125 &  N/A & N/A & N/A &N/A & N/A
\enddata
\end{deluxetable}

